SEA: Sentence Encoder Assembly for Video Retrieval by Textual Queries

Retrieving unlabeled videos by textual queries, known as Ad-hoc Video Search (AVS), is a core theme in multimedia data management and retrieval. The success of AVS counts on cross-modal representation learning that encodes both query sentences and videos into common spaces for semantic similarity computation. Inspired by the initial success of previously few works in combining multiple sentence encoders, this paper takes a step forward by developing a new and general method for effectively exploiting diverse sentence encoders. The novelty of the proposed method, which we term Sentence Encoder Assembly (SEA), is two-fold. First, different from prior art that use only a single common space, SEA supports text-video matching in multiple encoder-specific common spaces. Such a property prevents the matching from being dominated by a specific encoder that produces an encoding vector much longer than other encoders. Second, in order to explore complementarities among the individual common spaces, we propose multi-space multi-loss learning. As extensive experiments on four benchmarks (MSR-VTT, TRECVID AVS 2016-2019, TGIF and MSVD) show, SEA surpasses the state-of-the-art. In addition, SEA is extremely ease to implement. All this makes SEA an appealing solution for AVS and promising for continuously advancing the task by harvesting new sentence encoders.

==> infersent.tex <==
\textit{4) InferSent}. The traditional method of sentence coding is mainly unsupervised learning.
InferSent \cite{infersent} is a model of training with supervised learning methods, which has excellent performance in many natural language processing tasks.
Three computational operations are performed on sentence encoder with premise input and sentence encoder with hypothesis input to predict sentence relationships through a full connection layer and a softmax layer.

In our experiments, We use pre-training model that had been trained on SNLI(Stanford Natural Language Inference Datasets)\cite{SNLI}.SNLI consists of 570K sentence pairs labeled as entailment, contradiction and neutral. The task of training is to determine the label of each sentence pair. In the network structure of InferSent, the sentence encoder selects BiLSTM with Max pooling\cite{max_pooling} to generate vectors. Details are as follows, a sequence of P words \{$w_p$\}(p=1,...,P) trough words embedding get vector \{$v_p$\}(p=1,...,P) . For a more accurate expression of each word embeddings, we use opensource fastText vectors trained on Common Crawl 840B with 300 dimensions can dowload at https://dl.fbaipublicfiles.com/fasttext/vectors-english/crawl-300d-2M.vec.zip .Forward LSTM and bcakward LSTM respectively calculate \{$v_p$\} from two opposite directions ,then concatenate the results to get the vector \{$h_p$\} .The combination of these two structures in different directions is called BiLSTM\[v_p=fastText(w_1,...,w_P)\]\[f_p=Forward_pLSTM(v_1,...,v_P)\]\[b_p=Backward_pLSTM(v_1,...,v_P)\]\[h_p=[f_p,b_p]\]\[u=MaxPooling(h_p)\]The outputs \{u\} which dimension is 4096 is obtained by selecting the maximum value over each dimension of the hidden units(max poling) from BiLSTM . Pre-trained model(trained with fastText)  are available at https://dl.fbaipublicfiles.com/infersent/infersent2.pkl,the embedding vector of a whole sentence can be described as:\[\textbf{InferSent}(s) : = u\]


==> table-w2vvpp-avs.tex <==
\begin{table}[tb!]
\normalsize
\renewcommand\arraystretch{1.2}
\centering
\caption{\textbf{Performance of W2VV++ with varied setups in the TRECVID AVS tasks}, sorted in descending order by the mean performance.}
\label{tab:w2vv-avs}
\scalebox{0.82}{
\begin{tabular}{@{}|l | l | r | r | r |r | r | @{}}
\hline
\textbf{Video feature} & \textbf{Text encoder} & \textbf{TV16} & \textbf{TV17} & \textbf{TV18} & \textbf{TV19} & \textbf{Mean} \\
\hline
resnext-resnet&gru&0.124&0.165&0.082&0.075&0.112\\
\hline
resnet-152&w2v&0.122&0.163&0.089&0.101&0.119\\
\hline
resnet-152&gru&0.133&0.166&0.086&0.094&0.120\\
\hline
resnet-152&bow-w2v-gru&0.139&0.165&0.083&0.109&0.124\\
\hline
resnet-152&bow-gru&0.136&0.185&0.087&0.113&0.130\\
\hline
resnet-152&bow&0.125&0.193&0.091&0.115&0.131\\
\hline
resnext-101&w2v&0.123&0.181&0.112&0.115&0.133\\
\hline
resnet-152&bow-w2v&0.140&0.183&0.098&0.119&0.135\\
\hline
resnext-101&bow-w2v-gru&0.137&0.194&0.090&0.120&0.135\\
\hline
resnext-101&gru&0.142&0.195&0.096&0.121&0.138\\
\hline
resnext-resnet&w2v&0.131&0.190&0.113&0.126&0.140\\
\hline
resnext-101&bow-gru&0.144&0.194&0.101&0.133&0.143\\
\hline
resnext-101&bow-w2v&0.140&0.193&0.112&0.135&0.145\\
\hline
resnext-101&bow&0.148&0.200&0.109&0.140&0.149\\
\hline
resnext-resnet&bow-gru&0.154&0.214&0.101&0.136&0.151\\
\hline
resnext-resnet&bow-w2v&0.146&0.213&0.111&0.138&0.152\\
\hline
resnext-resnet&bow-w2v-gru&0.155&0.215&0.107&0.138&0.154\\
\hline
resnext-resnet&bow&0.156&0.218&0.110&0.151&0.159\\
\hline
\end{tabular}
}
\end{table}
